TAT-LLM: A Specialized Language Model for Discrete Reasoning over Tabular and Textual Data

In this work, we address question answering (QA) over a hybrid of tabular and textual data that are very common content on the Web (e.g. SEC filings), where discrete reasoning capabilities are often required. Recently, large language models (LLMs) like GPT-4 have demonstrated strong multi-step reasoning capabilities. We then consider harnessing the amazing power of LLMs to solve our task. We abstract a Step-wise Pipeline for tabular and textual QA, which consists of three key steps, including Extractor, Reasoner and Executor, and initially design an instruction to instantiate the pipeline and validate that GPT-4 outperforms all existing methods. However, utilizing an online LLM like GPT-4 holds various challenges in terms of cost, latency, and data security risk, which motivates us to specialize smaller LLMs in this task. We develop a TAT-LLM language model by fine-tuning LLaMA 2 with the training data generated automatically from existing expert-annotated datasets following the Step-wise Pipeline. The experimental results have verified that our TAT-LLM model can outperform all baseline models, including the previous best fine-tuned models and very large-scale LLMs like GPT-4 on FinQA, TAT-QA and TAT-DQA benchmarks.

==> 01_intro_bak.tex <==

In this work, we focus on analyzing a prevalent category of content in the real world, i.e. documents containing tables and text, including but not limited to SEC filings, academic papers, and medical reports. 
These documents often feature extensive numerical data in both tabular and textual formats, demanding discrete reasoning for intelligent comprehension.
Recent research~\cite{zhu2021tat,chen2021finqa} investigates the intelligent comprehension of such documents through question answering (QA) tasks, as exemplified in Figure~\ref{fig:sample}. 
The model, provided with a table and relevant text as the context, needs to perform various types of discrete reasoning, such as arithmetic calculations, making comparisons, and counting, to answer the question.


To perform QA over hybrid tabular and textual data, a straightforward approach~\cite{ran2019numnet,lei2022answering} involves taking the table, text, and question as input and generating the answer directly.
However, this approach can be ineffective due to the complex reasoning process involved~\cite{wei2022chain}. To address this, some works~\cite{Zhu2023SoarGraph,zhou2022unirpg} decompose the task into multiple steps, producing intermediate results that serve as references for the final answer. 
% For example, SoarGraph~\cite{Zhu2023SoarGraph} first extracts the relevant information by selecting nodes in a constructed table-text graph structure and then employs a tree-based method to explicitly generate the mathematical expression of the answer. 
These multi-step approaches typically require distinct modules for each step and often optimize them concurrently through multi-task learning. However, the problem of how to decompose and model the answer process remains an open challenge.


In this work, we identify three key steps in the process of tabular and textual QA, and abstract a \emph{Step-wise Pipeline}, as illustrated in \figref{qa_system} b).
In particular, 1) \textit{Extractor} identifies the relevant information or evidence to the question from the given context; 2) \textit{Reasoner} generates a mathematical equation or logic rule  with the obtained information; and 3) \textit{Executor} derives the final answer by executing the mathematical equation or logic rule with the associated information.
These three steps emphasize different abilities for tabular and textual QA  --- understanding of the question and context, knowledge (e.g., logic) of answering the question, and precision in calculating the answer.
As these steps produce a sequence of intermediate results, we can specifically model them and enhance their discrete reasoning ability given a practical scenario of tabular and textual QA problems.


The large language model (LLM) like ChatGPT~\cite{ouyang2023following} or FLAN~\cite{wei2022finetuned} has exhibited strong abilities required in the steps of the \emph{Step-wise Pipeline}, which are essentially emergent multi-step reasoning abilities~\cite{wei2022emergent} with proper instructions such as chain-of-thought (CoT)~\cite{wei2022chain} and least-to-most~\cite{zhou2023leasttomost}. 
We initially design a task instruction to instantiate the pipeline and validate it on GPT-4~\cite{openai2023gpt4}, showing promising results on multiple benchmarks. 
However, utilizing an online LLM presents challenges in terms of cost, latency, and data security risks. On the other hand, fine-tuning a smaller language model specifically for math word problems has proven fairly appealing~\cite{cobbe2021training,fu2023specializing}.
We are then motivated to explore the specialization of smaller language models for discrete reasoning over tabular and textual data following our abstracted \emph{Step-wise Pipeline}.


To this end, we develop a \model~model by fine-tuning LLaMA 2~\cite{touvron2023llama2} with the training data generated automatically from existing expert-annotated datasets, as shown in \figref{qa_system} c).
In particular, we train the selected LLM to take the table, text, and question as input, and complete the task in three steps following the \emph{Step-wise Pipeline}. 
We construct each of the training instances with five parts: Instruction, Table, Text, Question, and Response, from available tabular and textual QA datasets.
Inspired by Tab-CoT~\cite{ziqilu2023tabcot}, the model output (or response) is formatted to a structured table, with each row corresponding to one step of the pipeline, as shown in the right part of \figref{qa_system} c).
This design is friendly to further refining the final answer and automatic evaluation.
Moreover, to enhance the model performance, we equip the \model~model with an \emph{External Executor}, which strengthens the execution of logical rules and mathematical calculations to better infer the final answer.
We test our \model~on three popular benchmarks: FinQA~\cite{chen2021finqa}, TAT-QA~\cite{zhu2021tat} and TAT-DQA~\cite{zhu2022towards}.
The experimental results show that our smallest model \model~(7B) can outperform all baseline models and even beat GPT-4 on all three datasets. 
In summary, we make the following main contributions in this work:
\begin{itemize}[leftmargin=*]
    \item We abstract a \emph{Step-wise Pipeline} including \textit{Extractor}, \textit{Reasoner} and \textit{Executor} for better performing discrete reasoning and ground the pipeline on LLMs, showcasing their potential in the tabular and textual QA task.
    \item We develop a \model~model by fine-tuning LLaMA 2 for tabular and textual QA following the \emph{Step-wise Pipeline}, better supporting practical application with cost and privacy concerns. 
    \item We conduct extensive experiments on three popular benchmarks, validating the superiority of our \model~model over both conventional methods and very large-scale LMs, e.g. GPT-4.
\end{itemize}
